Do LLMs Understand Social Knowledge? Evaluating the Sociability of Large Language Models with SocKET Benchmark

Large language models (LLMs) have been shown to perform well at a variety of syntactic, discourse, and reasoning tasks. While LLMs are increasingly deployed in many forms including conversational agents that interact with humans, we lack a grounded benchmark to measure how well LLMs understand \textit{social} language. Here, we introduce a new theory-driven benchmark, SocKET, that contains 58 NLP tasks testing social knowledge which we group into five categories: humor & sarcasm, offensiveness, sentiment & emotion, and trustworthiness. In tests on the benchmark, we demonstrate that current models attain only moderate performance but reveal significant potential for task transfer among different types and categories of tasks, which were predicted from theory. Through zero-shot evaluations, we show that pretrained models already possess some innate but limited capabilities of social language understanding and training on one category of tasks can improve zero-shot testing on others. Our benchmark provides a systematic way to analyze model performance on an important dimension of language and points to clear room for improvement to build more socially-aware LLMs. The associated resources are released at https://github.com/minjechoi/SOCKET.

==> 2.obsolete.tex <==
\section{Comparing Model Capabilities via Few-shot Learning}
\label{sec:few-shot}
A major success factor of LLMs is the ability to finetune pretrained models to downstream tasks, which preserves both the pretrained language information as well as adapting to domain-specific settings. We can thus hypothesize that the social reasoning capabilities of LLMs also vary by the text corpus used for pretraining; i.e., models pretrained on text from more social settings should perform better than those trained on other genres. % We now turn our attention to identifying and comparing the level of social knowledge stored in identical models trained on different domain-specific datasets.
Therefore, we test multiple models whose parameters reflect diverse text used in pretraining in a few-shot setting to assess how pretrained text influences performance.
% Using a number of domain-specific LLMs trained on identical architectures, we compare their performances on social knowledge tasks when trained on \DATASET.

\myparagraph{Experimental Setup}
For each task, we generate five different samples of training sets with sample sizes of 50, 100, or 200. For imbalanced datasets (mostly binary tasks), we do upsampling to ensure that each label makes up at least 20\% of the sample. Details of how these training sets were constructed can be found in Appendix~(\sref{sec:appendix_data_processing}). We use four sets of parameters originating from the BERT~\citep{devlin2019bert} model: the original pretrained \texttt{bert-base-uncased} model and three variants obtained by training on legal documents~(\texttt{legalbert}~\citep{zheng2021legalbert}), science papers~(\texttt{scibert}~\citep{beltagy2019scibert}) and finance news ~(\texttt{finbert}~\citep{araci2019finbert}). We also include two parameter settings of the RoBERTa~\citep{liu2019roberta} model: the \texttt{roberta-base} model and a variant trained on tweets~(\texttt{twitter}~\citep{barbieri2020tweeteval}). Finally, we include a T5 model fine-tuned using fixed prompts. Training details and model parameters are listed in the Appendix~(\sref{sec:appendix_experiments})

\begin{figure}[t]
\centering
\includegraphics[width=0.5 \textwidth]{figures/few-shot-by-samples.pdf}
\caption{A comparison of pretrained LLMs on few-shot performances, trained on 50, 100, or 200 samples.}
\label{fig:fewshot-result}
\end{figure}

\myparagraph{Results}
We present the aggregated performances across tasks for the few-shot models trained on 50, 100, and 200 samples in Figure~\ref{fig:fewshot-result}~(see Figure~\ref{fig:fewshot-all} for detailed results). The addition of training samples in a few-shot learning setting improves performances across most settings, with the notable exception of \texttt{roberta-base}. Similar to Table~\ref{tab:benchmark_performance}, the prompt-based finetuning of T5 performs worse than its BERT-based counterparts. More importantly, we observe significant performance differences between models of the same size but trained on different text corpora. For instance, both \texttt{legalbert} and \texttt{scibert} consistently perform worse than \texttt{bert-base-uncased}, suggesting these models are pretrained on informative and factual text rather than conversations and social interactions. Meanwhile, \texttt{twitter} consistently outperforms \texttt{roberta-base}, which supports our hypothesis, given that not only do tweets are rich in emotions and social elements~\citep{kim2012twitter}. We conclude that an LLM's innate social understanding capability may differ depending on the richness of the social context it was pretrained on, and such differences can lead to further performance gaps when finetuned on downstream tasks that evaluate social knowledge.



\myparagraph{Cross Category Zeroshot Transfer}
% Different types of social information are interdependent and in this section, 
We further explore cross-category zeroshot learning for social knowledge. We fine-tune a \texttt{t5-base} model over datasets from each of the five categories using prompts and then evaluate their zero-shot performance on the remaining categories (cf. \sref{sec:appendix_experiments} for finetuning details). % We fine-tune separate t5-base models on each category of tasks and then evaluate each model on all the tasks. 
As shown in Figure \ref{fig:model_corr_category}, category-level fine-tuning tend to help other categories that are highly dependent on the trained category. For example, training on sentiment \& emotion data improves the zeroshot prediction of social factors and training on Humor \&  Sarcasm also helps to understand offensiveness. Such a result suggests that leveraging the task dependencies between social knowledge could help to build better NLP models for understanding social knowledge.

\begin{figure}[t]
% \centering
\includegraphics[width=0.49 \textwidth]{figures/t5_task_transfer.pdf}
\caption{Relative performance gain of the T5 model trained on each category of tasks. Knowledge learned from a certain social category can be transferred into other categories.}
\label{fig:model_corr_category}
\end{figure}


==> old_result_table.tex <==
\begin{table*}
\small
\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
\begin{center}
 \resizebox{0.99\textwidth}{!}{
\begin{tabular}{l r ccccc cccc c}
\toprule
category & \multicolumn{1}{c}{model}  &  Humor \& Sarcasm &  Offensiveness &  Sentiment \& Emotion &  Social Factors &  Trustworthiness &  CLS &  Classification &  PAIR &  Regression &  overall \\
\midrule
\multirow{2}{*}{Baseline} 
    & random &   0.50 & 0.39 & 0.36 & 0.41 & 0.40 & 0.42 & 0.39 &  0.52 & 0.11 & 0.41 \\
    & majority & 0.49 & 0.50 & 0.39 & 0.41 & 0.50 & 0.51 & 0.48 & 0.52 & 0.15 & 0.48 \\
\midrule
\multirow{4}{*}{Full data}
    & bert-base-uncased & 0.83 & 0.67 & 0.47 & 0.63 & 0.59 & 0.58 & 0.63 &  0.84 & 0.44 & 0.64 \\
    & roberta-base & & & & & &  & & & & \\
    & deberta-v3 &   0.83 &       0.67 &       0.47 &            0.63 &         0.59 & 0.58 &            0.63 &  0.84 &        0.44 &     0.64 \\
    & t5-full &   0.70 &       0.69 &       0.57 &            0.66 &         0.60 & 0.64 &            0.69 &   NaN &        0.32 &     0.65 \\
\midrule
% \multirow{3}{*}{Few-shot}
%     & bert-base-uncased & 0.83 & 0.67 & 0.47 & 0.63 & 0.59 & 0.58 & 0.63 &  0.84 & 0.44 & 0.64 \\
%     & roberta-base & & & & & &  & & & & \\
%     & t5-full &   0.70 &       0.69 &       0.57 &            0.66 &         0.60 & 0.64 &            0.69 &   NaN &        0.32 &     0.65 \\
% \midrule
\multirow{2}{*}{zeroshot} 
    & gpt2 &   0.39 &       0.43 &       0.24 &            0.34 &         0.38 & 0.38 &            0.40 &  0.31 &        0.12 &     0.37 \\
    & t5 &   0.34 &       0.37 &       0.24 &            0.30 &         0.47 & 0.40 &            0.34 &  0.34 &        0.13 &     0.36 \\
%\cline{1-12}
% \multirow{9}{*}{fewshot} 
%     & bert-base-uncased-fewshot-50 &   0.59 &       0.59 &       0.37 &            0.57 &         0.52 & 0.56 &            0.54 &  0.56 &        0.32 &     0.54 \\
%     & finbert-fewshot-50 &   0.58 &       0.59 &       0.39 &            0.57 &         0.53 & 0.56 &            0.56 &  0.53 &        0.27 &     0.55 \\
%     & legalbert-fewshot-50 &   0.56 &       0.58 &       0.33 &            0.55 &         0.53 & 0.55 &            0.54 &  0.54 &        0.28 &     0.53 \\
%     & majority-fewshot-50 &   0.33 &       0.46 &       0.19 &            0.30 &         0.46 & 0.44 &            0.38 &  0.34 &        0.06 &     0.39 \\
%     & random-fewshot-50 &   0.50 &       0.39 &       0.27 &            0.42 &         0.39 & 0.42 &            0.36 &  0.50 &        0.15 &     0.39 \\
%     & roberta-base-fewshot-50 &   0.60 &       0.61 &       0.37 &            0.54 &         0.53 & 0.54 &            0.59 &  0.55 &        0.30 &     0.56 \\
%     & scibert-fewshot-50 &   0.58 &       0.58 &       0.36 &            0.53 &         0.53 & 0.54 &            0.53 &  0.58 &        0.24 &     0.53 \\
%     & t5-fewshot-50 &   0.46 &       0.49 &       0.29 &            0.42 &         0.47 & 0.50 &            0.44 &  0.43 &        0.07 &     0.45 \\
%     & twitter-fewshot-50 &   0.64 &       0.61 &       0.41 &            0.61 &         0.54 & 0.57 &            0.59 &  0.56 &        0.30 &     0.57 \\
%\cline{1-12}
\bottomrule
\end{tabular}

}
\end{center}
    \caption{A comparison on the benchmark performances of different models and training schemes}
    \label{tab:benchmark_performance}
\end{table*}

